Characterizations of periods of multidimensional shifts

We show that the sets of periods of multidimensional shifts of finite type (SFTs) are exactly the sets of integers of the complexity class $\NE$. We also show that the functions counting their number are the functions of #E. We also give characterizations of some other notions of periodicity. We finish the paper by giving some characterizations for sofic and effective subshifts.

==> notations.tex <==
% divers
\renewcommand{\mid}{\;\middle\vert\; }
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\id}{\mathop{\mathrm{id}}\nolimits}
\newcommand{\tr}{\mathop{\mathrm{tr}}\nolimits}

% ensembles
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\NN}{\ensuremath{\mathbb{N}}}
\newcommand{\QQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\cantor}{\ensuremath{\left\{0,1\right\}^\NN}}
\newcommand{\fullshift}{{\Sigma^{\ZZ^d}}}

\newcommand{\norminf}[1]{\|#1\|_\infty}
\newcommand{\abs}[1]{|#1|}

% calculabilité

\newcommand{\sizu}{\ensuremath{\Sigma^0_1}\xspace}

\newcommand{\halts}[2][truie]{\ifthenelse{\equal{#1}{truie}}{#2\!\downarrow}{#2\!\downarrow^{#1}}}
\newcommand{\haltsnot}[1]{{#1\!\uparrow}}

\newcommand{\pb}[1]{\textsc{#1}\xspace}
\newcommand{\cofin}{\pb{COFIN}}
\newcommand{\finite}{\pb{FIN}}
\newcommand{\total}{\pb{TOTAL}}

%sous-shifts

\newcommand{\boule}[1]{{\mathcal{B}_{#1}}}


\newcommand{\subshift}[1]{{\mathcal{X}_{#1}}}
\newcommand{\forbid}{{\mathcal F}}
\newcommand{\tuile}[1]{\protect\tikz[scale=0.3,baseline={([yshift=-4pt]current bounding
box.center)}]{\protect\draw[color=gridcolor,fill=#1] (0,0)
rectangle +(1,1);}\xspace}
\newcommand{\motifdeux}[2]{{\protect\tikz[scale=0.3]{
  \protect\draw[color=gridcolor,fill=#1] (0,0) rectangle +(1,1);
  \protect\draw[color=gridcolor,fill=#2] (1,0) rectangle +(1,1);
}}}
\newcommand{\admissible}[2]{{\mathcal{A}_{#1}\left(#2\right)}}
\newcommand{\extensible}[2]{{\mathcal{E}_{#1}\left(#2\right)}}
\newcommand{\card}[1]{{\##1}}
\newcommand{\taille}[1]{{\left|#1\right|}}

% périodicité
\newcommand{\strongper}[1]{{\mathfrak{P}_{#1}}}
\newcommand{\oneper}[1]{{\mathfrak{P}^1_{#1}}}
\newcommand{\kper}[2]{{\mathfrak{P}^{#1}{#2}}}
\newcommand{\horper}[1]{{\mathfrak{P}^h_{#1}}}
\newcommand{\nbper}[2]{{\mathfrak{N}_{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}}
\newcommand{\recper}[1]{{\mathfrak{P}^r_{#1}}}
\newcommand{\lattice}{\Gamma}

% complexité
\newcommand{\un}[1]{un\left(#1\right)}
\newcommand{\bin}[1]{bin\left(#1\right)}
\newcommand{\bigO}[1]{\ensuremath{\mathcal O\left(#1\right)}}

\usepackage[bold,basic]{complexity}






==> texcommands.tex <==
\colorlet{gridcolor}{black}
%% Symboles de SFTs
\newcommand{\sbreaker}{\fill[color=black] (0.375,0) rectangle (0.625,1);}
\newcommand{\breaker}{\tikz[scale=0.25]{\sbreaker}\xspace}
\newcommand{\shorline}{\fill[color=black] (-0.5,0) rectangle (0.5,0.25);}
\newcommand{\horline}{\tikz[scale=0.25]{\shorline}\xspace}
\newcommand{\shempty}{\draw[color=black] (-0.5,0) -- (0.5,0);}
\newcommand{\hempty}{\tikz[scale=0.25]{\shempty}\xspace}
\newcommand{\scorner}{
  \fill[color=black] (0.375,0) rectangle (0.625,1);
  \fill[color=black] (0,0.375) rectangle (1,0.625);
}
\newcommand{\corner}{\tikz[scale=0.25]{\scorner}\xspace}
\newcommand{\ssepa}{\fill[color=black] (0,0) rectangle (0.75,0.75);}
\newcommand{\sepa}{\tikz[scale=0.25]{\ssepa}\xspace}

%%% Symboles pour la diagonale
\colorlet{leftcolor}{yellow}
\colorlet{rightcolor}{red}
\newcommand{\sdiagdiag}{
\fill[color=leftcolor](0,0) -- (1,1) -- (0,1) -- cycle;
\fill[color=rightcolor](0,0) -- (1,1) -- (1,0) -- cycle;
}
\newcommand{\sdiagleft}{
\fill[color=leftcolor](0,0) rectangle  (1,1);
}
\newcommand{\sdiagright}{
\fill[color=rightcolor](0,0) rectangle (1,1);
}
\newcommand{\sdiaghor}{
\fill[color=leftcolor](0,0) rectangle (1,0.5);
\fill[color=rightcolor](0,0.5) rectangle (1,1);
}
\newcommand{\sdiagver}{
\fill[color=leftcolor](0.5,0) rectangle (1,1);
\fill[color=rightcolor](0,0) rectangle (0.5,1);
}
\newcommand{\sdiagcorner}{
\fill[color=rightcolor](0,0) rectangle (1,1);
\fill[color=leftcolor](0.5,0) rectangle (1,0.5)  (0.5,0.5) -- (1,1) -- (0.5,1) -- cycle (0,0) -- (0.5,0.5) -- (0,0.5) -- cycle;
}
\newcommand{\diagcorner}{\tikz[scale=0.25]{\sdiagcorner}\xspace}
\newcommand{\diagver}{\tikz[scale=0.25]{\sdiagver}\xspace}
\newcommand{\diaghor}{\tikz[scale=0.25]{\sdiaghor}\xspace}
\newcommand{\diagright}{\tikz[scale=0.25]{\sdiagright}\xspace}
\newcommand{\diagleft}{\tikz[scale=0.25]{\sdiagleft}\xspace}
\newcommand{\diagdiag}{\tikz[scale=0.25]{\sdiagdiag}\xspace}


\newcommand\cube[4]{
 \begin{scope}[shift={(#4)}]
  \begin{scope}[every node/.append style={yslant=0.5},yslant=0.5]
   \begin{scope}
    #2
   \draw (0,0) rectangle +(1,1);
   \end{scope}
  \end{scope}
  \begin{scope}[shift={(0,1)},every node/.append style={yslant=0.5,xslant=-1},yslant=0.5,xslant=-1]
   \begin{scope}[shift={(0,1)},rotate=-90]
    #3
   \draw (0,0) rectangle +(1,1);
   \end{scope}
  \end{scope}
  \begin{scope}[shift={(-1,0.5)},every node/.append style={yslant=-0.5},yslant=-0.5]
   \begin{scope}
    #1
   \draw (0,0) rectangle +(1,1);
   \end{scope}
  \end{scope} 
 \end{scope}
}


